Understanding (Non-)Robust Feature Disentanglement and the Relationship Between Low- and High-Dimensional Adversarial Attacks

Recent work has put forth the hypothesis that adversarial vulnerabilities in neural networks are due to them overusing "non-robust features" inherent in the training data. We show empirically that for PGD-attacks, there is a training stage where neural networks start heavily relying on non-robust features to boost natural accuracy. We also propose a mechanism reducing vulnerability to PGD-style attacks consisting of mixing in a certain amount of images contain-ing mostly "robust features" into each training batch, and then show that robust accuracy is improved, while natural accuracy is not substantially hurt. We show that training on "robust features" provides boosts in robust accuracy across various architectures and for different attacks. Finally, we demonstrate empirically that these "robust features" do not induce spatial invariance.

==> Experimentssettings.tex <==
\section{Experimental Setting}

==> old_tables.tex <==
\begin{table}[htb]
    \caption{Accuracies achieved from the experiments described in Section. The first row of the table contains natural accuracies, while the remaining rows contain robust accuracies under the attack mentioned in the leftmost column. Each model has four columns of results: ``$D$'' refers to models trained with the natural dataset, while ``$D_R$'' refers to models trained with the robust dataset. The notation $^*$ indicates the model is trained with \texttt{std*} data augmentation} \label{tab:spatialattack_all}
    \begin{adjustwidth}{-.5in}{-.5in}  
        \vspace{15pt}
        \begin{center}
            \begin{tabular}{|c|cccc|cccc|cccc|c|}
                \hline
                & \multicolumn{4}{c|}{ResNet-50} & \multicolumn{4}{c|}{G-ResNet-18} & \multicolumn{4}{c|}{G-ResNet-34} & PTN \\
                Attack & $D$ & $D_R$ & $D^*$ & $D_R^*$ & $D$ & $D_R$ & $D^*$ & $D_R^*$ & $D$ & $D_R$ & $D^*$ & $D_R^*$ & STN\footnotemark \\ 
                \hline
                None &
                94.84 & 84.75 & 93.9 & 83.53 &  % ResNet-50
                94.66 & 85.46 & 94.74 & 85.11 &  % G-ResNet
                \textbf{95.72} & 84.93 & 94.72 & 84.55 &  % STN
                -- \\
                \texttt{rot10} &
                80.97 & 67.78 & 83.24 & 69.67 &  % ResNet-50
                83.27 & 69.22 & 87.42 & 72.98 &  % G-ResNet
                83.56 & 68.8 & \textbf{87.61} & 73.34 &  % STN
                -- \\
                \texttt{rot30} &
                36.77 & 24.94 & 58.75 & 42.62 &  % ResNet-50
                41.74 & 26.95 & 69.86 & 51.97 &  % G-ResNet
                41.07 & 26.08 & \textbf{75.38} & 46.47 &  % STN
                -- \\
                \texttt{grid775,10$^\circ$} &
                63.34 & 52.3 & 67.78 & 55.31 &  % ResNet-50
                68.17 & 54.24 & \textbf{75.7} &  % G-ResNet
                58.96 & 67.98 & 55.15 & \textbf{75.7} & 60.38 &  % STN
                -- \\
                \texttt{grid135} &
                18.72 & 11.23 & 39.71 & 26.89 &  % ResNet
                21.84 & 11.81 & 52.51 & 36.64 &  % G-ResNet
                20.99 & 10.99 & \textbf{56.06} & 31.52 &  % STN
                -- \\
                \texttt{grid775} &
                15.28 & 9.88 & 35.42 & 24.53 &  % ResNet
                19.36 & 10.78 & 49.69 & 34.57  % G-ResNet
                & 17.82 & 9.89 & \textbf{53.19} & 29.78 &  % STN
                -- \\
                \hline
            \end{tabular}
        \end{center}
    \end{adjustwidth}
    \vspace{-15pt}
\end{table}
